A Physics-Informed Neural Network-Based Approach for the Spatial Upsampling of Spherical Microphone Arrays

Spherical microphone arrays are convenient tools for capturing the spatial characteristics of a sound field. However, achieving superior spatial resolution requires arrays with numerous capsules, consequently leading to expensive devices. To address this issue, we present a method for spatially upsampling spherical microphone arrays with a limited number of capsules. Our approach exploits a physics-informed neural network with Rowdy activation functions, leveraging physical constraints to provide high-order microphone array signals, starting from low-order devices. Results show that, within its domain of application, our approach outperforms a state of the art method based on signal processing for spherical microphone arrays upsampling.

==> results/nmse_channels.tex <==
\begin{tikzpicture}%
\begin{axis}[%
    xlabel={Number of available channels},%
    ylabel={$\mathrm{NMSE}$},%
    y unit = \decibel, %
    ytick = {-12, -8, -4, 0},
    xtick = data,
    symbolic x coords={4,9,16,25},
    % xmin=196, xmax=5000,
    % ymax=0, ymin=-45,
    axis x line=bottom,%
    axis y line=left, %
    grid, %
    height=5.5cm, %
    width=\columnwidth, %
    enlarge x limits=0.08,%
    enlarge y limits=0.08,%
    % style={scale=0.5, transform shape, font=\tiny}
    style={font=\normalsize},%
    legend columns=2,%
    legend style={at={(0.38,0.05)},anchor=south,font=\small},%
    log ticks with fixed point,
    legend cell align={left}
]

\addplot[mark=triangle, line width=0.3mm] table {results/nmse_channels_sarita.txt};%
\addlegendentry{Sarita}%

% \addplot[dashed, line width=0.3mm] table {results/nmse_channels_siren.txt};%
% \addlegendentry{SIREN} %

% \addplot[dashdotted, line width=0.3mm] table {results/nmse_channels_siren_pde.txt};%
% \addlegendentry{SIREN + PDE}%

\addplot[mark=o, line width=0.3mm] table {results/nmse_channels_siren_pde_rowdy.txt};%
\addlegendentry{Proposed} %

\end{axis}%
\end{tikzpicture}

==> results/nmse_freq_4.tex <==
\begin{tikzpicture}%
\begin{axis}[%
    xlabel={Frequency},%
    ylabel={\(\text{NMSE}_f \)},%
    y unit = \decibel,
    x unit = \kilo\hertz,
    xticklabels={0,0,2,4,6,8},
    % xmin=196, xmax=5000,
    ymin=-20,
    ymax=5,
    axis x line=bottom,%
    axis y line=left, %
    grid, %
    height=4cm, %
    width=\columnwidth, %
    enlarge x limits=0.08,%
    enlarge y limits=0.08,%
    % style={scale=0.5, transform shape, font=\tiny}
    style={font=\normalsize},%
    legend columns=2,%
    legend style={at={(0.95,0.05)},anchor=south east,font=\small},%
    log ticks with fixed point,%
    legend cell align={left}
]

\addplot[line width=0.3mm, orange] table {results/nmse_freq_proposed.txt};%
\addlegendentry{Proposed}%
\addplot[line width=0.3mm, blue] table {results/nmse_freq_sarita.txt};%
\addlegendentry{SARITA}%

\end{axis}%
\end{tikzpicture}

==> results/nmse_freq_9.tex <==
\begin{tikzpicture}%
\begin{axis}[%
    xlabel={Frequency},%
    ylabel={\(\text{NMSE}_f \)},%
    y unit = \decibel,
    x unit = \kilo\hertz,
    xticklabels={0,0,2,4,6,8},
    % xmin=196, xmax=5000,
    ymin=-20,
    ymax=5,
    axis x line=bottom,%
    axis y line=left, %
    grid, %
    height=4cm, %
    width=\columnwidth, %
    enlarge x limits=0.08,%
    enlarge y limits=0.08,%
    % style={scale=0.5, transform shape, font=\tiny}
    style={font=\normalsize},%
    legend columns=2,%
    legend style={at={(0.95,0.05)},anchor=south east,font=\small},%
    log ticks with fixed point,%
    legend cell align={left}
]

\addplot[line width=0.3mm, orange] table {results/nmse_freq_proposed_9.txt};%
\addlegendentry{Proposed}%
\addplot[line width=0.3mm, blue] table {results/nmse_freq_sarita_9.txt};%
\addlegendentry{SARITA}%

\end{axis}%
\end{tikzpicture}
